Label Distribution Shift-Aware Prediction Refinement for Test-Time Adaptation

Test-time adaptation (TTA) is an effective approach to mitigate performance degradation of trained models when encountering input distribution shifts at test time. However, existing TTA methods often suffer significant performance drops when facing additional class distribution shifts. We first analyze TTA methods under label distribution shifts and identify the presence of class-wise confusion patterns commonly observed across different covariate shifts. Based on this observation, we introduce label Distribution shift-Aware prediction Refinement for Test-time adaptation (DART), a novel TTA method that refines the predictions by focusing on class-wise confusion patterns. DART trains a prediction refinement module during an intermediate time by exposing it to several batches with diverse class distributions using the training dataset. This module is then used during test time to detect and correct class distribution shifts, significantly improving pseudo-label accuracy for test data. Our method exhibits 5-18% gains in accuracy under label distribution shifts on CIFAR-10C, without any performance degradation when there is no label distribution shift. Extensive experiments on CIFAR, PACS, OfficeHome, and ImageNet benchmarks demonstrate DART's ability to correct inaccurate predictions caused by test-time distribution shifts. This improvement leads to enhanced performance in existing TTA methods, making DART a valuable plug-in tool.

==> table_cifar10.tex <==
% \begin{table}[!t]
%     \centering
%     \caption{Average accuracy on CIFAR-10C/10.1-imb. \textbf{Bold} indicates the best performance for each benchmark.
%     The prediction refinement of DART consistently contributes to effective adaptation combining with existing TTA methods.
%     }
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lccccc|ccccc}
%     \toprule
%         ~ & \multicolumn{5}{c|}{CIFAR-10C} & \multicolumn{5}{c}{CIFAR-10.1}  \\ 
%         ~ & \multicolumn{5}{c|}{Imbalance ratio (IR)} & \multicolumn{5}{c}{Imbalance ratio (IR)}  \\ 
%         ~ & 1 & 5 & 20 & 50 & 5000 & 1 & 5 & 20 & 50 & 5000  \\ \midrule
%         NoAdapt & 0.7162 & 0.7169 & 0.7167 & 0.7164 & 0.7168 & 0.8745 & 0.8738 & 0.8742 & 0.8744 & 0.8748  \\ \midrule
%         BNAdapt \cite{bnadapt_schneider} & 0.8530 & 0.7715 & 0.4997 & 0.3464 & 0.2033 & 0.8570 & 0.7756 & 0.5110 & 0.3595 & 0.2107  \\ 
%         \rowcolor{Gray}
%         BNAdapt+ours & 0.8536 & 0.8160 & 0.7372 & 0.7582 & 0.8168 & 0.8571 & 0.8117 & 0.7315 & 0.7450 & 0.8092  \\ \midrule
%         TENT \cite{tent_wang} & 0.8647 & 0.7578 & 0.4729 & 0.3263 & 0.1908 & 0.8548 & 0.7426 & 0.4682 & 0.3268 & 0.1982  \\ 
%         \rowcolor{Gray}
%         TENT+ours & 0.8716 & 0.8113 & 0.7169 & 0.7720 & 0.8697 & 0.8607 & 0.8033 & 0.7040 & 0.7402 & 0.8458  \\ \midrule
%         PL \cite{pseudolabel_lee} & 0.8652 & 0.7693 & 0.4854 & 0.3339 & 0.1944 & 0.8585 & 0.7700 & 0.4823 & 0.3349 & 0.1968  \\ 
%         \rowcolor{Gray}
%         PL+ours & 0.8616 & 0.8082 & 0.7214 & 0.7682 & 0.8468 & 0.8612 & 0.8029 & 0.7096 & 0.7486 & 0.8249  \\ \midrule
%         ODS \cite{ods_zhou} & 0.8613 & 0.8221 & 0.6814 & 0.6064 & 0.5411 & 0.8568 & 0.8111 & 0.6701 & 0.5868 & 0.5080  \\ 
%         \rowcolor{Gray}
%         ODS+ours & 0.8566 & 0.8316 & 0.8066 & 0.8355 & 0.8607 & 0.8557 & 0.8180 & 0.7954 & 0.8260 & 0.8505  \\ \midrule
%         SAR \cite{sar_niu} & 0.8530 & 0.7715 & 0.4997 & 0.3464 & 0.2033 & 0.8547 & 0.7754 & 0.5112 & 0.3585 & 0.2109  \\ 
%         \rowcolor{Gray}
%         SAR+ours & 0.8536 & 0.8160 & 0.7372 & 0.7582 & 0.8168 & 0.8549 & 0.8117 & 0.7304 & 0.7454 & 0.8099  \\ \midrule
%         LAME \cite{lame_boudiaf}& 0.8533 & 0.7869 & 0.5300 & 0.3772 & 0.2319 & 0.8524 & 0.7880 & 0.5387 & 0.3844 & 0.2358  \\ 
%         \rowcolor{Gray}
%         LAME+ours & 0.8532 & 0.8022 & 0.6754 & 0.7396 & 0.8818 & 0.8522 & 0.8023 & 0.6744 & 0.7233 & 0.8636  \\ \midrule
%         DELTA \cite{delta_zhao}& 0.8610 & 0.8375 & 0.7338 & 0.6651 & 0.5942 & 0.8515 & 0.8307 & 0.7345 & 0.6719 & 0.5947  \\ 
%         \rowcolor{Gray}
%         DELTA+ours & 0.8666 & 0.8656 & 0.8328 & 0.8366 & 0.9245 & 0.8591 & 0.8564 & 0.8374 & 0.8249 & 0.9165  \\ \midrule
%         NOTE \cite{note_gong}& ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ &   \\ 
%         \rowcolor{Gray}
%         NOTE+ours & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ &   \\ 
%         \bottomrule
%     \end{tabular}
%     }
% \end{table}

==> table_pacs.tex <==
\begin{table}[!t]
    \centering
    \caption{Average accuracy on PACS and OfficeHome. \textbf{Bold} indicates the best performance for each benchmark. DART enhances the performance combined with existing entropy minimization-based TTA methods. Refer to Appendix~\ref{appendix: full_results} for the combined results with other TTA methods.
    }
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccccccccccc|c}
    \toprule
        \multicolumn{14}{c}{PACS}\\ \midrule
        Method & a2c & a2p & a2s & c2a & c2p & c2s & p2a & p2c & p2s & s2a & s2c & s2p & avg  \\ \midrule
        NoAdapt & 66.0+-0.0 & 97.8+-0.0 & 57.3+-0.0 & 75.6+-0.0 & 90.2+-0.0 & 72.2+-0.0 & 73.2+-0.0 & 39.7+-0.0 & 43.9+-0.0 & 23.5+-0.0 & 50.3+-0.0 & 38.0+-0.0 & 60.7+-0.0  \\ \midrule
        BNAdapt & 75.8+-0.3 & 97.0+-0.2 & 70.0+-0.2 & 82.5+-0.3 & 95.1+-0.4 & 73.5+-0.7 & 77.8+-0.2 & 65.0+-0.4 & 46.9+-0.2 & 59.4+-0.5 & 69.0+-0.4 & 57.8+-0.2 & 72.5+-0.0  \\ 
        \rowcolor{Gray}
        BNAdapt+ours & 76.0+-0.3 & 96.8+-0.1 & 72.1+-0.5 & 84.4+-0.6 & 95.4+-0.2 & 74.7+-0.3 & 76.1+-0.3 & 62.0+-0.4 & 55.0+-0.7 & 74.1+-0.2 & 76.7+-0.2 & 74.0+-0.6 & 76.4+-0.1  \\ \midrule
        TENT & 78.6+-0.9 & 97.8+-0.5 & 77.1+-1.9 & 88.0+-0.3 & 97.1+-0.5 & 79.1+-1.2 & 81.7+-0.6 & 75.5+-1.0 & 59.2+-2.5 & 60.1+-1.1 & 71.0+-1.0 & 56.8+-1.6 & 76.8+-0.6  \\ 
        \rowcolor{Gray}
        TENT+ours & 80.8+-0.8 & 97.7+-0.4 & 79.2+-0.7 & 88.9+-0.2 & 97.4+-0.3 & 79.2+-1.2 & 79.6+-1.0 & 75.4+-1.7 & 69.8+-1.5 & 81.3+-0.6 & 77.6+-0.7 & 71.6+-0.5 & 81.6+-0.4  \\ \midrule
        DELTA & 79.6+-1.0 & 98.5+-0.2 & 75.4+-2.2 & 89.3+-0.2 & 97.8+-0.2 & 80.9+-1.2 & 82.3+-0.5 & 77.4+-1.4 & 62.5+-0.9 & 60.6+-1.8 & 72.0+-1.1 & 62.2+-5.0 & 78.2+-0.6  \\ 
        \rowcolor{Gray}
        DELTA+ours & 81.7+-1.1 & 98.3+-0.1 & 77.0+-1.3 & 89.8+-0.3 & 97.7+-0.2 & 80.5+-1.6 & 79.5+-1.2 & 76.7+-0.9 & 66.6+-1.8 & 83.6+-0.4 & 76.7+-2.1 & 71.8+-1.1 & \textbf{81.7+-0.4}  \\ \midrule
        \multicolumn{14}{c}{OfficeHome}\\ \midrule
        Method & a2c & a2p & a2r & c2a & c2p & c2r & p2a & p2c & p2r & r2a & r2c & r2p & avg  \\ \midrule
        NoAdapt & 47.9+-0.0 & 65.8+-0.0 & 73.2+-0.0 & 52.4+-0.0 & 63.2+-0.0 & 64.2+-0.0 & 49.8+-0.0 & 46.3+-0.0 & 71.8+-0.0 & 65.2+-0.0 & 51.7+-0.0 & 77.5+-0.0 & 60.8+-0.0  \\  \midrule
        BNAdapt & 48.2+-0.1 & 62.4+-0.2 & 71.4+-0.2 & 51.2+-0.3 & 62.6+-0.2 & 62.9+-0.1 & 51.3+-0.1 & 48.3+-0.4 & 72.3+-0.4 & 64.5+-0.4 & 53.6+-0.5 & 76.3+-0.2 & 60.4+-0.1  \\ 
        \rowcolor{Gray}
        BNAdapt+ours & 47.8+-0.3 & 63.5+-0.1 & 72.4+-0.2 & 52.7+-0.4 & 63.2+-0.2 & 63.7+-0.2 & 51.9+-0.3 & 48.9+-0.2 & 72.8+-0.4 & 64.5+-0.4 & 53.8+-0.4 & 76.8+-0.2 & 61.0+-0.1  \\  \midrule
        TENT & 48.1+-0.4 & 62.0+-0.8 & 69.5+-0.6 & 54.6+-0.4 & 63.7+-0.7 & 64.3+-0.8 & 52.2+-0.3 & 47.7+-0.7 & 72.3+-0.5 & 65.5+-0.7 & 54.0+-0.6 & 76.6+-0.4 & 60.9+-0.2  \\ 
        \rowcolor{Gray}
        TENT+ours & 49.8+-0.4 & 65.3+-0.5 & 71.4+-0.4 & 55.8+-0.5 & 65.0+-0.6 & 65.7+-0.4 & 53.3+-0.4 & 48.4+-0.4 & 72.8+-0.3 & 66.0+-0.6 & 54.8+-0.7 & 77.2+-0.4 & 62.1+-0.2  \\  \midrule
        DELTA & 50.6+-0.6 & 65.6+-0.4 & 72.3+-0.4 & 56.3+-0.9 & 67.1+-0.7 & 66.8+-0.1 & 52.8+-0.7 & 49.9+-0.4 & 74.7+-0.2 & 66.6+-1.0 & 56.7+-0.5 & 78.1+-0.3 & 63.1+-0.1  \\ 
        \rowcolor{Gray}
        DELTA+ours & 51.5+-0.4 & 67.6+-0.2 & 73.6+-0.3 & 57.4+-0.5 & 67.4+-0.6 & 67.6+-0.6 & 54.2+-0.4 & 50.1+-0.6 & 75.1+-0.1 & 66.9+-0.7 & 56.9+-0.7 & 78.3+-0.1 & \textbf{63.9+-0.1}  \\ 
        \bottomrule
    \end{tabular}
    }
    \label{table: pacs}
\end{table}

